Long-tailed Extreme Multi-label Text Classification with Generated Pseudo Label Descriptions

Extreme Multi-label Text Classification (XMTC) has been a tough challenge in machine learning research and applications due to the sheer sizes of the label spaces and the severe data scarce problem associated with the long tail of rare labels in highly skewed distributions. This paper addresses the challenge of tail label prediction by proposing a novel approach, which combines the effectiveness of a trained bag-of-words (BoW) classifier in generating informative label descriptions under severe data scarce conditions, and the power of neural embedding based retrieval models in mapping input documents (as queries) to relevant label descriptions. The proposed approach achieves state-of-the-art performance on XMTC benchmark datasets and significantly outperforms the best methods so far in the tail label prediction. We also provide a theoretical analysis for relating the BoW and neural models w.r.t. performance lower bound.

==> tex/abstract_introduction.tex <==
\begin{abstract}
% v1
% Extreme multi-label text classification (XMTC) is 
% the task of tagging each document with the relevant labels in a large set of predefined labels. 
% Most of the state-of-the-art (SOTA) models simply treat each label as an index whose embedding is randomly initialized. 
% Due to the highly skewed label distribution, a majority of the labels (namely the tail labels) receive very few training instances, posing a hard optimization problem of those label embeddings via supervised signals.
% While other works leverage the label side information, they assume that the document and label descriptions are strongly related.
% However, we observe that in real datasets, the label descriptions are usually very short, noisy, and nonspecific to the document. 
% Since obtaining high quality label descriptions for a large number of labels is both expensive and impractical, we propose to extract keywords from the label embedding of a trained sparse classifier as pseudo label descriptions. 
% We then apply a dual encoder framework to leverage the correlation between the document and the pseudo label description to enhance existing classification system. We prove both theoretically and empirically that our framework brings improvement to the XMTC benchmark datasets, especially on the tail label prediction.

% v2
Extreme multi-label text classification (XMTC) is 
the task of tagging each document with the relevant labels in a large predefined label space, where the label frequency distribution is often highly skewed.  That is, a large portion of labels (namely the tail labels) have very few positive instances, posing a hard optimization problem for training the classification models.  The severe data sparse issue with tail labels is more announced in recent neural classifiers, where the embeddings of both the input documents and the output labels need to be jointly learned, and the success of such learning relies on the availability of sufficient training instances. This paper addresses this tough challenge in XMTC by proposing a novel approach that combines the strengths of both traditional bag-of-words (BoW) classifiers and recent neural embedding-based classifiers.  Specifically, we use a trained BoW model to generate a pseudo description for each label, and apply a neural model to establish the mapping between input documents and target labels in the latent embedding spaces. Our experiments show significant improvements of the proposed approach over other strong baseline methods on benchmark datasets, especially on tail label prediction. We also provide a theoretical analysis for relating BoW and neural models w.r.t. performance lower bound.
%Due to the highly skewed label distribution, a majority of the labels (namely the tail labels) receive very few training instances, posing a hard optimization problem for machine learning.
%The state-of-the-art (SOTA) neural models typically employ a pre-trained Transformer as feature extractor whose parameters are jointly optimized with the label embeddings. 
%We argue that the joint optimization paradigm may be suboptimal especially for tail labels, which receive an overwhelming amount of negative instances. As a result, neither the feature nor the label embeddings are sufficiently optimized.
%While other works leverage the label side information, they assume that the document and label descriptions are strongly related.
%To alleviate the problem, we complement the neural model with a trained sparse classifier. 
%Specifically, we propose to extract keywords from the label embedding of a trained sparse classifier as pseudo label descriptions.
%We then apply a dual encoder framework to leverage the correlation between the document and the pseudo label description to enhance existing classification system. 
%We prove both theoretically and empirically that our framework brings improvement to the XMTC benchmark datasets, especially on the tail label prediction.

%Current models jointly train document and label embeddings, and then use the inner product to produce a relevance score. 
%As majority of the labels are assigned with very few training instances in the XMTC problem, 

%The most challenging part of the problem is due to a highly skewed label distribution where the majority of the categories (namely the tail labels) have very few training instances. 
\end{abstract}

\section{Introduction}
Extreme multi-label text classification (XMTC) is the task of tagging each document with the relevant category labels in a very large predefined label space, in which the number of categories can be from a few thousands to more than a million. It has a wide range of potential applications, such as assigning subject topics to articles, tagging keywords for online shopping recommendation, classifying products for tax purposes, and so on.

\begin{figure}[th!]
     \centering
     \includegraphics[width=\linewidth]{img/data_dist.png}
     \caption{In the skewed distribution of XMTC, tail labels with less than $10$ training instances cover a large portion, if not the majority, of the label space, but their training instances cover a only small percentage of the training set.}
     \label{fig:data_dist}
\end{figure}

%In the target space of XMTC problems, 
The label frequencies in XMTC often follow a power law. That is, a small portion of the labels have a dominating number of training instances (namely head labels), whereas the majority of the labels have very few training instances (namely as tail labels), as illustrated in \figref{fig:data_dist}. The severe data sparse issue with the tail labels poses a harder optimization problem for XMTC than the  classification tasks where the number of categories are much smaller and the label distributions are not as skewed.

%A classification system typically consists of two components: 1) a feature extractor that converts each input document into feature vector, and 2) a classifier with \yy{a vector of model parameters per label (wich can be viewed as label embedding pf that label). The system can be optimized %by a point-wise with a loss function such as the Binary Cross Entropy (BCE) per label.} %We argue that this pipeline maybe suboptimal for the XMTC under the extremely skewed distribution where tail labels are negative labels for a large number of instances.

%Traditional classification systems adopt the bag-of-words feature extractor that captures the corpus specific word importance statistics such as tf-idf. 
Traditional classifiers typically use a bag-of-words (BoW) vector to represent each document, whose dimension is the the entire document vocabulary.  Each word in the document is treated as an one-hot vector weighted by the tf-idf~\cite{kuang2010improvement} value. Summing over the one-hot vectors of the within-document words yields the BoW representation of the document. Since the BoW vectors of documents are typically high-dimensional and very sparse, we call the classification models based on such representation as BoW classifiers or \textit{sparse classifiers}. 
Models like DiSMEC~\cite{babbar2017dismec}, ProXML~\cite{babbar2019proxml} and PPDSparse~\cite{yen2017ppdsparse} are recent examples of this kind.
%optimize sparse label embeddings efficiently via the one-vs-all (OVA) methods. 
BoW classifiers enjoy their simplicity and effectiveness in utilizing local and global frequencies of words in unlabeled data, such as TF (the within-document frequency of each word) and IDF (the within-corpus inverted document frequency of each word), which is arguably a strength in addressing the severe data sparse issue in tail label prediction (see the rest of this paper for deeper insights).  As for their weaknesses or limitations, the word independence assumption in the BoW presentations is clearly unjustified, as word location, ordering and semantic dependencies in context are ignored. %the sparse features 
%suffer from several limitations such as ignoring the word location or the lack of semantic information.

In contrast, recent neural classifiers use %deep learning models employ 
neural networks to extract latent features with learnable parameters, and obtain a lower dimensional dense vector as document embedding. Typically, neural classifiers learn the latent label embeddings jointly with the document embeddings in an end-to-end training process. Since the learned document and label representations are both dense vectors, we call such models \textit{dense classifiers} in this paper. %with semantic information. 
%With the advances of transfer learning techniques, l
Recently, large pre-trained Transformer-based models such as BERT~\cite{devlin2018bert} and XLNet~\cite{yang2019xlnet} have been adapted to XMTC problems to extract expressive contextualized features. Examples include  X-Transformer~\cite{chang2020taming}, APLC-XLNet~\cite{ye2020pretrained} and LightXML~\cite{jiang2021lightxml}, which achieved state-of-the-art (SOTA) performance on several benchmark datasets for XMTC evaluation. Despite the desirable expressiveness of such dense classifiers, how much does their successes depend on the availability of a large quantity of labeled training data, and how much does their performance suffers under severe data sparse conditions?  These questions have not investigated in sufficient depth so far. Furthermore, the dense classifiers do not make explicit use of the unsupervised statistics like tf-idf term weights, which maybe a potential weakness. 

%Although jointly optimizing the feature extractor and label embedding brings more flexibility, we argue that this pipeline maybe suboptimal for the extremely skewed distribution in XMTC where a large amount of tail labels receive very few positive instances.

%According to our analysis, the learning of label embedding and feature embedding influences each other such that, in one step of gradient decent, the label embedding is an aggregation of feature embedding, and vice versa. However, the overwhelming number of negative instances for a tail label cause disruptive effect in both feature and label embedding learning, making the classification system perform poorly on the tail labels. In other words, neither the feature nor the label embedding can be sufficiently optimized by the joint optimization paradigm.

This paper aims to improve the prediction power of XMTC classifiers especially with respect to tail label prediction. Specifically, we propose a framework that combines the strengths of both BoW sparse classifiers and neural dense classifiers. The key idea is 1) using a trained BoW model to select keywords for each label, which yields the pseudo label description, and 2) training a neural model based on the training pairs of input documents and the pseudo descriptions.  Step 1 leverages the strength of Bow models in using unsupervised TF-IDF statistics, which would be particularly important under severe data sparse conditions (see \secref{sec:rethinking} for details) , and Step 2 takes advantage of a neural encoder in learning expressive representations (embeddings) of documents and labels. Our experiments show significant improvements of the proposed approach over other strong baseline methods on benchmark datasets, especially on tail label prediction. A theoretical analysis is also provided for relating BoW and neural models w.r.t. performance lower bound.
%In this paper, we propose to alleviate the above problem by leveraging a trained sparse classifier for two reasons: 1) the sparse tf-idf feature is unsupervised and doesn't need to be jointly optimized with the label embedding. 2) the learned sparse label embedding encodes the token importance information, which can be a good resource for learning label embedding in neural models. Therefore, we design a Keyword-selected Dual Encoder (\ourmodelshort) framework. Specifically, we select keywords from a trained sparse classifier as pseudo label description, and then apply a dual encoder to leverage the relation between the document and label description. 
%We prove theoretically that our model can achieve a lower bound performance as the sparse classifier and demonstrate the effectiveness of our model on XMTC benchmark datasets, especially on the tail label prediction.
%However, since most of the instance are negative for a tail label, the it has a disruptive effect during learning. As a result, the tail label cannot be sufficiently optimized. 



%Recently, deep Transformer-based models have achieved the state-of-the-art (SOTA) performance on XMTC. Typically, those classification systems consist of two modules: 1) a feature extractor that converts the input text into a dense vector embedding, and 2) a logistic regression classifier with label embeddings as parameters. The two modules are jointly optimized by the binary cross entropy (BCE) loss. We argue that this pipeline maybe suboptimal for the XMTC under the extremely skewed distribution where tail labels are negative labels for a large number of instances.

%According to our analysis, on the feature extractor side, the learned document features are biased towards the head label representations and lack for the tail label representations; on the label embedding side, the tail labels are hard to encode any distinctive feature into the embeddings. 
%We propose to reduce the learning bias in the first problem with the unsupervised sparse feature (tf-idf) and alleviate the second problem with additional information on the label side to initialize the label embedding. Both aspects are addressed in our proposed Keyword-selected Dual Encoder (\ourmodelshort) framework. Specifically, we extract the pseudo label description from a trained sparse classifier, and apply a dual encoder to leverage the relation between the document and label description. We prove theoretically that our model achieves a lower bound performance as the sparse classifier.

%Although previously X-Transformer \citep{chang2020taming} has explored combining sparse feature with neural feature, it simply concatenates the tf-idf feature with the learned neural embedding to train a ranker, which is mathematically equivalent to adding the prediction scores of two independent systems. In other words, it is not using the tf-idf feature to enhance the neural model. 

%The recently proposed SiameseXML \cite{dahiya2021siamesexml} is related to our work, as it leverages the label description for enhanced multi-label classification, but it assumes that the input text and the label descriptions are strongly related to each other. However, most of the descriptions in real dataset are short, noisy and non-specific to the corpus, making it hard to be understood without further definition. 
%Since relying on human to provide high quality labels for the large output space is unrealistic, we propose a cheaper yet effective method to generate pseudo label description that can be fed into a deep neural network model for enhanced generalization. 

%we propose to extract pseudo label description by selecting keywords from a trained sparse model.

%Our key contributions are summarized as the follows: 1) We analyze the difficulty of optimization feature extractor and label embedding under skewed distribution. 2) We propose to alleviate the problem by generating corpus specific pseudo label description used by a dual encoder, which shows superior performance especially on tail label prediction. 3) We analyze theoretically the lower bound performance of the dual encoder with respect to the sparse classifier.


%As an example, in the Wiki-31K benchmark dataset shown in \figref{fig:data}, only $1\%$ of labels has more than $100$ training instances, but they cover more than $40\%$ of all the training instances. On the other hand, $89\%$ of labels only cover less than $30\%$ of training instances. Other benchmark datasets show similar distribution (Appendix \ref{sec:append_data}).


% It is worth pointing out that the performance of current SOTA models has been evaluated using the micro-averaging precision scores as the dominating metric~\cite{liu2017deep, you2018attentionxml, ye2020pretrained, chang2020taming, jiang2021lightxml}. %Since the micro-based precision 
% This metric gives an equal weight to the score of each instance when computing the average performance on a test set.  As a result, the global average is dominated by the system's performance on head labels. In other words, such a metric is not sufficiently sensitive for evaluating the performance of methods in tail label prediction, and possibly misleading in method comparison.
% Furthermore, metrics with a single score prohibit a fine-grained analysis of model performance with respect to the different label frequencies. 


% In order to assess the true success of the current SOTA methods in XMTC on tail label prediction, we present a re-examination of them by our proposed \textit{binned macro-averaging F1 metric}. Specifically, the labels are binned according to their training frequencies and the performance score of each label is given an equal weight when calculating the average over all labels in the bin.

% By comparing a set of SOTA neural models with a binary Support Vector Machines (SVM) as a  baseline on several benchmark datasets, we reveal that the deep-layered pre-trained Transformer models~\cite{ye2020pretrained, jiang2021lightxml, chang2020taming} perform worse than the simple SVM baseline in tail label prediction, while a label-word attention-based RNN model~\cite{you2018attentionxml}  outperformed the SVM baseline on two of those benchmark datasets.







==> tex/background.tex <==
\section{Background}
% We will introduce the notation and formulation in Section \ref{sec:background_intro}, the SOTA methods under evaluation in Section \ref{sec:background_methods} and the evaluation metrics in Section \ref{sec:background_metric}. 

\subsection{Preliminary}
%\section{One-vs-all Multi-label Classification}
%We will introduce the task and notation in Section \ref{sec:background_intro}, the SOTA methods under evaluation in Section \ref{sec:background_methods} and the evaluation metrics in Section \ref{sec:background_metric}. 

Let $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ be the training data where $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
%
The XMTC method can be formulated as learning a scoring function $f(\mathbf{x}, l) \in \sR$ defined on an input and candidate label pair $(\vx, l)$. The score should be higher for relevant labels than irrelevant labels.
The objective function of a classification model is defined as:
%Then we can define a classification model with the following objective function:
%The one-vs-all classifiers is optimized by:
\begin{equation*}
        \min_{f} \quad \frac{1}{N_{\text{train}} L} \sum_{i=1}^{N_{\text{train}}} \sum_{l=1}^{L} \mathcal{L}(y_{i l}, f(\mathbf{x}_i, l))
\end{equation*}
where $\mathcal{L}(\cdot, \cdot)$ is an instance-wise loss, such as a hinge loss in a Linear SVM or a sigmoid loss in the final layer of a neural network.

In the evaluation, since multi-labels can be relevant for an input document $\mathbf{x}$, a typical way is to measure the quality of a top-k ranked list of the predicted label: \begin{equation}
    \operatorname{Top-k}([f(\vx, 1), \ldots, f(\vx, L)])
\end{equation}
% \begin{equation*}
%         \mathbf{p}^k = \operatorname{Top-k}([f(\mathbf{x}, 1), \ldots, f(\mathbf{x}, L)])
% \end{equation*}


% We should add to related work later
%Although these approaches achieve good performance, with the enormous label space, these methods suffer from huge computational burden.As a remedy, Tree-based approaches are proposed ~\cite{fastxml,parabel,khandagale2019bonsai} to partition the labels into several clusters hierarchically based on their positive instances or correlations.Cluster-level classifiers are trained at each tree layer, which allows prediction in a hierarchical order. Many recent neural models are built upon tree-based methods, in which $f$ is neural networks.


\subsection{Tf-idf+SVM vs. Dense Neural Model} 
\noindent \textbf{Tf-idf+SVM} The one-vs-all linear SVM model is a simple realization of $f(\mathbf{x}, l)$:
\begin{equation*}
    f(\vx, l) = \langle \phi_t(\vx), \vw_l \rangle 
\end{equation*}
where $\phi_{\text{t}}(\vx) \in \sR^{v}$ converts each text input into the tf-idf feature with vocabulary size of $v$, and $\vw_l \in \mathbb{R}^v$ is the learned parameter of linear classifier for label $l$. The tf-idf feature uses the human defined heuristics to reflect the distributed importance of each word in the training corpus. 

%Although more complicated kernels such as the RBF kernel are introduced in the SVM model for the classification tasks, \cite{chang2011libsvm} shows that a Linear SVM achieves the same performance with a RBF kernel SVM when the feature space is large (refer to Table \ref{tab:dataset} for the number of features in the benchmark datasets). 
%Therefore, we use the Linear SVM to lower computational cost without affecting the performance. 


The document-vector representation-based methods (\textit{doc-vec}) encodes the raw text into a dense vector representation with neural networks as $\phi_n(\vx)$. %shown in Fig~\figref{fig:method} left.
%Specifically, \citet{liu2017deep} are the first to apply CNN model~\cite{kim-2014-convolutional} to encode the input text $\mathbf{x}$ into a single bottleneck vector as the document-level representation in the XMTC task. Recently, the deep Transformer-based~\cite{NIPS2017_3f5ee243} models quickly exceed the performance of CNN and achieve the state-of-the-art. We choose the deep Transformer-based models and write score function as follows:
\begin{equation}
    f(\vx, l) = \langle \phi_n(\vx), \vu_l \rangle 
\end{equation}
where $\phi_n(\vx) \in \sR^{d}$ is a $d$ dimensional dense feature usually obtained by the deep transformer models such as BERT~\citep{devlin2018bert} or XLNet~\citep{yang2019xlnet}. 
$\vu_l$ represents the learned parameter of a linear classifier for label $l$, which is typically optimized by the logistic regression objective $\mathcal{L}_{\mathrm{logistic}}$. We use $\vu_l$ to distinguish from $\vw_l$ because $\vu_l \in \sR^d$ is a compressed dense vector while $\vw_l \in \sR^v$ is sparse ($d \ll v$).
%From another point of view, it computes the similarity between the document vector and label embeddings as a score for the label. 
%The predicted labels are ranked according to the probability, and the top labels are compared against the ground truth label list. 

The most representative deep Transformer-based models tailored for the XMTC task are  X-transformer~\cite{chang2020taming}, APLC-XLNet~\cite{ye2020pretrained} and LightXML~\cite{jiang2021lightxml}, which are discussed in Appendix~\ref{sec:append_experiment}.



==> tex/experiment.tex <==
\section{Experiments}
\label{sec:experiment}

\begin{table*}[t!]
    \small
    \centering
    \begin{tabular}{l|cccccccc}
    \toprule
    Dataset & $N_{train}$ & $N_{test}$ & $F$ & $\bar{L}_d$ & $L$ & $p_{\text{tail}}^l$ & $p_{\text{tail}}^d$ \\
    \midrule
    EURLex-4K & 15,539 &  3,809 & 34,932 & 5.30 & 3,956 & 63.48\% & 9.50\% \\
    Wiki10-31K & 14,146 & 6,616 & 189,795 & 18.64 &  30,938 & 88.65\% & 27.06\%  \\
    AmazonCat-13K & 1,186,239 & 306,782 & 200,000 & 5.04 & 13,330 & 29.53\% & 0.27\% \\
    \bottomrule
    \end{tabular}
    \caption{$N_{\text{train}}$ and $N_{\text{test}}$ are the number of training and testing instances respectively. $F$ is the tf-idf feature size. $\bar{L}_d$ is the average number of labels per document. $L$ is the number of labels. For tail labels with $1\sim 9$ training instances, $p_{\text{tail}}^l$ is percentage of tail labels and $p_{\text{tail}}^d$ is the percentage of training instances covered by the tail labels. \label{tab:dataset}} 
\end{table*}

\begin{table*}[ht!]
    \centering
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{3}{c}{EUR-Lex} &  \multicolumn{3}{c}{Wiki10-31K} & \multicolumn{3}{c}{AmazonCat-13K} \\
    \midrule
    Methods & P@1 & P@3 & P@5 & P@1 & P@3 & P@5 & P@1 & P@3 & P@5\\
    \midrule
    DisMEC  &  83.21 & 70.39 & 58.73 & 84.13 & 74.72 & 65.94 & 93.81 & 79.08 & 64.06 \\
    PfastreXML & 73.14 & 60.16 & 50.54 &  83.57 & 68.61 & 59.10 & 91.75 & 77.97 & 63.68 \\
    Parabel & 82.12 & 68.91 & 57.89 & 84.19 & 72.46 & 63.37 & 93.02 & 79.14 & 64.51 \\
    Bonsai & 82.30 & 69.55 & 58.35 &  84.52 & 73.76 & 64.69 &  92.98 & 79.13 & 64.46 \\
    \midrule
    AttentionXML & 85.12 & 72.80 & 61.01  & 86.46 & 77.22 & 67.98  & 95.53 & 82.03 & 67.00 \\
    X-Transformer & 85.46 & 72.87 & 60.79 & 87.12 & 76.51 & 66.69 & 95.75 & 82.46 & 67.22 \\
    BERT-APLC & 85.54 & 72.68 & 60.59 & 88.54 & 77.21 & 67.43 & 94.49 & 79.74 & 64.46\\
    XLNet-APLC & 86.83 & 74.34 & 61.94 & 88.99 & 78.79 & 69.79 & 94.56 & 79.78 & 64.59\\
    LightXML & 86.12 & 73.87 & 61.67 & 87.39 & 77.02 & 68.21 & 94.61 & 79.83 & 64.45\\
    \midrule
    tf-idf+SVM (ours)  & 83.44 & 70.62 & 59.08 & 84.61 & 74.64 & 65.89 & 93.20 & 78.89 & 64.14 \\
    BERT (ours) & 84.72 & 71.66 & 59.12 & 87.60 & 76.74 & 67.03 & 94.26 & 79.63 & 64.39 \\
KDE & 86.13 & 73.82 & 62.22 & 88.52 & 78.13 & 68.98 &  96.13 & \bf 82.70 & \bf 67.52 \\
KDE+SVM & \bf 87.98 & \bf 75.81 & \bf 63.62  & \bf 89.10 & \bf 80.24 & \bf 70.49 & \bf 96.25 & 81.90 & 65.20 \\
    \bottomrule
    \end{tabular}
    \caption{Comparisons between \ourmodel and the SOTA sparse and dense classifiers. The results are evaluated with the micro-averaging P@5 metrics, with highest values in bold. We report our baseline sparse (tf-idf+SVM) and dense (BERT) classifiers with KDE and KDE+SVM (average of KDE and SVM predicted score).}
    \label{tab:micro_all}
\end{table*}

\subsection{Experimental Setting}
\paragraph{Datasets}
We conduct our experiments on $3$ benchmark datasets: EURLex-4K~\citep{10.1007/978-3-540-87481-2_4}, Wiki10-31K~\citep{zubiaga2012enhancing} and AmazonCat-13K~\citep{10.1145/2507157.2507163}.
The statistics of the datasets are shown in Table~\ref{tab:dataset}.
For the tail label evaluation, we consider the labels with $1 \sim 9$ training instances, because we assume the absolute number of training instance reflects the difficulty of optimization across datasets. The tail labels covers $63.48\%$, $88.65\%$ and $30\%$ of training labels for the $3$ datasets respectively. 
We obtain the datasets from the Extreme classification Repository\footnote{\url{http://manikvarma.org/downloads/XC/XMLRepository.html}} and a unstemmed version of EURLex-4K from the APLC-XLNet github\footnote{\url{https://github.com/huiyegit/APLC_XLNet.git}}.
% \begin{figure*}[ht!]
%      \centering
%      \includegraphics[width=0.45\linewidth]{img/eurlex_bin1.png}
%      \includegraphics[width=0.45\linewidth]{img/wiki10_bin1.png}
%      \includegraphics[width=0.48\linewidth]{img/amazoncat_bin1.png}
%      \includegraphics[width=0.48\linewidth]{img/amazoncat_bin2.png}
%      \caption{Comparison of the word-label attention-based method and the document vector-based method with different layers of BERT model on the benchmark datasets. The relative improvement to SVM on macro-averaging F1 is plotted.}
%      \label{fig:attn_cls_layers}
% \end{figure*}
%From the evaluations in the previous sections, we observe that the deep Transformer-based models achieves the best on the micro-based metrics, while the AttentionXML model achieves the best results on the tail label prediction on the two benchmark datasets. 
%Our hypothesis is that the deep Transformer models are powerful at exploiting the global semantic meaning because they are initialized with the general language knowledge from large text corpus via unsupervised pretraining. On the other hand, the word-label attention method in the AttentionXML exploits the less abstract semantics such as the word embedding features that may benefit tail label prediction when training instances are scarce. 
%A natural question is that whether we can combine the two to use the word-label attention to leverage the word knowledge in the pretrained model, and thus achieving consistent improvement on tail label prediction over all the benchmark datasets.

%Inspired by the observation of previous section, we try to leverage the less abstract features such as word-level features for tail label prediction.
%To this end, we propose to apply the word-label attention on the BERT model to integrate the word knowledge into the word-label matching process. We show that this method can achieve consistent improvement on tail label predictions.
\paragraph{Implementation Details} For the sparse model, since the public available BoW feature doesn't have a vocabulary dictionary, we generate the tf-idf feature by ourselves. We tokenize and lemmatize the raw text with the Spacy~\cite{spacy2} library and extract the tf-idf feature with the Sklearn~\cite{scikit-learn} library, with unigram whose idf is $>= 2$ and $<= 70\%$. For the dense model, we fine-tune a $12$ layer BERT-base model with different learning rates for the BERT encoder, BERT pooler and the classifier. The learning rates are $(1e-5$, $1e-4$, $1e-3)$ for Wiki10-31K and $(5e-5$, $1e-4$, $2e-3)$ for the rest datasets. We used learning rate $1e-5$ for fine-tuning the \ourmodel model. For the pseudo label descriptions, we concatenate the provided label description with the generated the top $20$ keywords. The final length is truncated up to $32$ after BERT tokenization.

\paragraph{Evaluation Metrics}
We use the micro-averaging $P@k$ metric to evaluate the overall system performance and the macro-averaging $F1@k$ metric to evaluate the tail label prediction, because both precision and recall are important for tail label predictions (and $F1@k$ is a harmonic average of both).

\noindent \textbf{micro-averaging P@k:} 
The micro-averaging P@k metric is widely used to evaluate a ranked list of predicted labels:
\begin{equation}
    P@k = \frac{1}{k} \sum_{i=1}^{k} \mathbbm{1}_{\vy_i^+}(p_i)
\end{equation}
where  $p_i$ is the $i$-th label in the predicted ranked list $\vp$ and $\mathbbm{1}_{\vy_i^+}$ is the indicator function. The metric score is averaged over all the test instances.

\noindent \textbf{macro-averaging F1@k:}
The $F1$ metric is a harmonic average of prediction (P) and recall (R):
\begin{equation}
    \operatorname{F1} = 2 \frac{P \cdot R }{P + R }
\end{equation} 
The precision and recall for a predicted ranked list $\vp$ are computed by $\mathrm{P}= \frac{\mathrm{TP}}{\mathrm{TP} + \mathrm{FP}}, \mathrm{R}=\frac{ \mathrm{TP}}{ \mathrm{TP} + \mathrm{FN}}$ according to the confusion matrix in \tblref{tab:confusion_matrix}.
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{4pt}
    \small
    \begin{tabular}{c|cc}
    & $l$ in $\vy_i$ & $l$ not in $\vy_i$ \\
    \hline
    $l$ in $\vp_i$ & True Positive($\mathrm{TP}_l^i$) & False Positive($\mathrm{FP}_l^i$) \\
    $l$ not in $\vp_i$ & False Negative($\mathrm{FN}_l^i$) & True Negative($\mathrm{TN}_l^i$) \\
    \end{tabular}
    \caption{Confusion Matrix for instance $i$ and label $l$ given the ranked list $\vp_i$.}
    \vspace{-1.0em}
    \label{tab:confusion_matrix}
\end{table}

Given $N_{\text{test}}$ instances and $L$ labels, the macro-average computes the scores on individual category first ($\mathrm{F1}_l$), and then take an average over all the categories ($\mathrm{F1} = \frac{1}{|\sL|}\sum_{i \in \sL} \mathrm{F1}_l$), which reflects label level performance of the methods.

For micro-averaging P@k, we choose $k=1,3,5$ the same as in other works. For macro-averaging F1@k, we choose $k=19$ for Wiki10-31K because it has an average of $18.64$ labels and $k=5$ for the rest datasets.


\paragraph{Baselines}
Our method is compared with the state-of-the-art baselines including both the sparse and dense classifiers. Specifically, DisMEC~\cite{babbar2017dismec}, PfastreXML~\cite{jain2016extreme}, Parabel~\cite{prabhu2018parabel}, Bonsai~\cite{khandagale2019bonsai} belong to the sparse classifiers, and X-Transformer~\cite{chang2020taming}, APLC-XLNet~\cite{ye2020pretrained} and LightXML~\cite{jiang2021lightxml}, AttentionXML~\cite{you2018attentionxml} belong to the dense classifier. X-Transformer, LightXML, and APLC-XLNet employ pre-trained Transformers to encode a document into a fixed embedding. We report the single model performance (chosen from their papers) with BERT-large for X-Transformer, BERT-base for LightXML and XLNet-base for APLC-XLNet. The AttentionXML utitizes label-word attention to generate label-aware word embedding instead of a fix document representation. We provide an additional linear SVM model with our extracted tf-idf features as a sparse baseline, and BERT-base classifier as a dense baseline.


\subsection{Experimental Results and Discussions} 
The performance of model evaluated on the micro-averaging P@5 metric is reported in \tblref{tab:micro_all}. 

\noindent \textbf{Sparse and dense classifiers:} The sparse classifiers (first panel) generally underperform the dense models (second panel) under the micro-averaging evaluation metric. Our implementation of Linear SVM model and BERT model achieve comparable result with the sparse and dense classifiers respectively, except that the AttentionXML and X-Transformer achieve better result in Amazoncat-13K. The reason could be that the Amazoncat-13K product categorization relies more on the lexicon matching features, which gives the two methods performance gains. 

\noindent \textbf{\ourmodelshort:} Our KDE model is fine-tuned on top of the BERT model with the pseudo label descriptions generated from the SVM model. As shown in the result, \ourmodel has additional gains on both of the classifiers, indicating \ourmodel can: 1) leverage the keyword semantic from sparse model for better generalization, 2) alleviate the difficult of optimization of neural model with scarce data by providing label side information. The KDE model outperforms the baseline models on the Amazoncat-13K dataset, and the KDE+SVM (average of KDE and sparse classifier scores) performs the best on the other two datasets. 


\begin{figure}[th!]
     \centering
     \includegraphics[width=\linewidth]{img/tail_label.png}
     \caption{The evaluation of tail label prediction for a dense classifier base (BERT) and our proposed \ourmodel with different settings. The metric is  macro-averaging F1@k, where $k=19$ for Wiki10-31K and $k=5$ for the other datasets. The figure shows the relative improvement to the SVM baseline with $*$ indicating the significance for $p<0.01$.}
     \label{fig:macro_tail}
\end{figure}
\subsection{Tail Label Evaluation} 
Previously, we observe that the pre-trained Transformer-based models underperform the sparse classifier (Linear SVM baseline) on tail label prediction. In this section, we want to test the ability of \ourmodel to generalize over the sparse classifier with the generated pseudo label description for tail label prediction. The experimental results are shown in \figref{fig:macro_tail}, where we report the relative performance of the models under investigation with respect to the sparse classifier. Specifically, we include the dense classifier (BERT) without any label side information as a baseline, which underperforms the SVM on all of the datasets. 

\noindent \textbf{Only Provided Label Text} We fine-tune \ourmodel with only the provided label text, denoted as \ourmodel+label. The model outperforms the sparse classifier on the EURLex-4K and Amazoncat-13K dataset, with the latter one being significant. This is probably because these two datasets has higher quality label text compared with Wiki10-31K, where the label space is both large and noisy.

\noindent \textbf{Pseudo Label Description} We fine-tune \ourmodel with pseudo label descriptions, denoted as \ourmodel+label+key$k$, where $k$ is the length of the pseudo label description after BERT tokenization. We observe that with keyword length $16$, the model performs the best, which achieves significant improvement on the tail label prediction for all datasets. With larger $k=32$ in the default setting, the model includes additional "less important" keywords, which may introduce noises and thus lower the performance.

% \subsection{Ablation Study}
% We conduct an ablation study with different number of keywords selected and show the performance respectively.
%From the observation of previous section, we find that attentionXML achieves the best performance among all the baselines on tail labels prediction.
%This observation inspires us to combine the AttentionXML model with pre-trained Transformers.
% In the word-label attention, each label attends to the contextualized word embedding to select the most relevant information from each word, which more efficiently utilizes the local word features. Specifically, the contextualized word embeddings $\mathbf{h}$ in Eq.(\ref{eq:attn_xml}) are the outputs from a neural model and each label integrates the most relevant $\mathbf{h}$ to form the feature embedding in Eq.(\ref{eq:attn_xml2}). The final score function is calculated by Eq.(\ref{eq:attn_xml3}).

% To obtain the contextualized word embedding, the AttentionXML uses a $1$ layer bi-directional RNN model. In a pretrained Transformer model, there are $12$ layers for BERT-Base and $24$ layers for BERT-Large, and different layers may encode different level syntactic or semantic features~\cite{jawahar:hal-02131630}. Therefore, we explore the effect of using different layers of Transformer models with either word-label attention or typical the document-vector representation-based methods in the next section.



% \subsection{Experiments with Shallow and Deep BERT Models}
% %Using deeper pre-trained Transformers achieves better performance on most of the downstream tasks~\cite{devlin2018bert}.
% In this section, we show the performance of tail label prediction by controlling the number of layers for BERT by $[1, 2, 4, 6, 12]$ for both the word-label attention method (\textit{word-label}) and the document-vector representation-based method (\textit{doc-vec}). For "$k$ layer(s) BERT", we simply use the first $k$ layer(s) of BERT, discarding the remaining top layers. The models are trained on the full training data, and the relative improvement over the SVM baseline is reported on the tail labels ($[1\sim 9]$ for EURLex-4K and Wiki10-31K, $[1\sim 9], [10\sim 99]$ for AmazonCat-13K). The results of model performance are shown in Figure \ref{fig:attn_cls_layers} and more evaluations are shown in Appendix \ref{tab:shallow_transformer}.

% In the results, we have two key conclusions 1) the word-label methods perform the better with shallower BERT models and the doc-vec methods perform better with deeper BERT models, and 2) the shallow BERT model with $1$ or $2$ layers show consistently improvement over the SVM baseline on tail label predictions. 
%Note that all the SOTA deep Transformer-based model underperform the SVM baseline in the bins evaluated. Therefore, our word-label BERT method improves from the current SOTA Transformer-based models.


% The results also align with our hypothesis. For deeper Transformer models, the input tokens interact with each others via self-attention, gradually forming more complex and abstract semantic representations from layer to layer.
% Hence, the representations of the top layer encode the global document semantic.
% On the other hand, the shallower Transformer models reflect more of the token level meaning with only a little context information. The stronger word-level feature can help the word-label attention better leverage the local information for enhanced tail label prediction.

% Our findings raise an interesting point that most of the pretrained models use the [CLS] embedding as a default and the local feature of Transformer models in bottom layers are often ignored, but they can be potentially beneficial for different tasks.

% In addition to the improvement in tail label prediction, the shallower Transformer model has fewer number of parameters, which makes the training and inference much faster.

%question that whether using deeper Transformers is always better when the training instances are insufficient.

% The "doc-vec" denotes the document vector based method, which uses the [CLS] embedding as the single of an entire document, while in "word-label attn", each label selects the most relevant word as its unique document representation.

\begin{comment}

\section{Experiments}
\label{sec:experiment}
In our experiments, we probe which Transformer architecture can benefit tail label prediction, which is evaluated by proposed binned macro-based F1.
Also, we analyze the performance of the document representation-based method versus the label attention-based method.

\subsection{Datasets}
\label{sec:dataset}
We use three benchmark datasets: EUR-Lex (4K), Wiki10-31K and AmazonCat-13K.

\subsection{Shallow vs. Deep Transformers}
In the Transformer models, each word interacts with each other using self-attention, gradually forming more abstract representations from layer to layer.
Hence, the embeddings of the last layer encodes the richest semantic meaning of the entire document, which are usually used as the document representation.
In XMTC, recent works extract document representation by pooling over the last layer's embedding~\cite{chang2020taming,ye2020pretrained}, or concatenating the [CLS] embeddings from the last few layers to collect more semantic information\cite{jiang2021lightxml}.

As mentioned in the previous section, less abstract level features are potentially suitable for tail label prediction.
Intuitively, deeper Transformer layers encode the high-level semantic information~\cite{tenney-etal-2019-bert}.
Hence, the first architecture design that we want to explore is the depth of the Transformer model.
For different model depths, we control the number of layers for BERT by $[1, 2, 4, 6, 12]$ layers.



As shown in Fig \ref{fig:attn_cls}, we observe that using shallow layers of BERT benefits label attention-based method, while deep Transformer benefits the document representation-based method. 
This can be expected because the Transformer model gradually refines the latent embedding of each word by incorporating more context information via the self-attention mechanism over the layers. 
Compared with the upper layers, the word identity will be overwritten by the contextualized information. 
Therefore, word level retrieval-based method will perform worse on the upper layers. To the contrary, as more contextualized information is injected into the [CLS] embedding in the upper layers, the global information helps document embedding to encode useful feature for the label classification. 

From Table \ref{tab:results}, the performance of the retrieval-based method and the representation-based method are similar, with the retrieval-based method slightly better on P@1 and the representation-based method better on P@5. However, the two models are based on really different feature and underlying mechanism, so we will compare the difference in the next part.

\subsection{Comparison with Baselines}

In this Section, we compare our proposed AttentionXL+BERT with other baselines.


%The results are shown in Fig. \ref{fig:bin}. The horizontal axis represents the label bins according to the number of training instances and the groups are $\{1\sim9, 10\sim 99, \ldots \}$. The vertical axis represents the relative improvement compared with the flat svm baseline. From the figure, we observe that retrieval-based method benefits the lower-frequency (tail) bins, and the representation-based method benefits the high-frequency (head) bins. As most of the training instances concentrate in the head bins, the micro precision metric will be largely impacted by the prediction in those groups. Therefore, the advantage of the retrieval method in the tail bins is shadowed by the micro P@k metric. Especially in the Wiki10-31K dataset, although retrieval based method performs worse on the precision metric, it has a huge advantage on the prediction of tail labels.





%Roughly (may elaborate), the training time for $1$ layer retrieval-based model is $2$ mins per epoch and for $12$ layers document representation-based model is $9$ mins per epoch, so the light weight retrieval is $4.5$ times faster.

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{c|ccc}
%     & p1 & p3 & p5 \\
%     SVM & 83.44 & 70.62 & 59.08 \\
%     X-Transformer & 85.46 & 72.87 & 60.79 \\
%     BERT-APLC & 85.54 & 72.68 & 60.59 \\
%     XLNet-APLC  & 86.83 & 74.34 & 61.94 \\
%     LightXML & 86.12 & 73.87 & 61.67 \\
%     % attn & 86.59 & 73.21 & 60.90 \\
%     % cls 12 & 85.64 &  73.57 &  61.20\\
%     %ensemble & 87.77 & 75.73 & 63.08 \\
%     % average & 88.14 & 75.77 & 63.36 \\
%     % rank &  87.80 & 75.69 & 63.29 \\
%     % roundrobin & 86.59 & 74.62 & 62.28 \\
%     \end{tabular}
%     \caption{Baseline results on EUR}
%     \label{tab:results}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{c|ccc}
%     & p1 & p3 & p5 \\
%     SVM & 84.61 & 74.64 & 65.89 \\
%     X-Transformer & 87.12 & 76.51 & 66.69 \\
%     BERT-APLC & 88.54 & 77.21 & 67.43 \\
%     XLNet-APLC & 88.99 & 78.79 & 69.79 \\
%     LightXML  & 87.39 & 77.02 & 68.21 \\
%     % attn 1 & 83.80 & 73.71 & 64.78 \\
%     % cls 12 & 88.42 & 77.04 & 66.88 \\
%     % average &  89.08 &  79.17 &  69.75 \\
%     % rank &  88.61 &  78.57 &  68.98 \\
%     % roundrobin &  83.80 &  76.72 &  67.83 \\
%     %ensemble & 89.08 & 79.24 & 69.86 \\
%     \end{tabular}
%     \caption{Baseline results on Wiki10}
%     \label{tab:results}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{c|ccc}
%     & p1 & p3 & p5 \\
%     SVM & 93.20 & 78.89 & 64.14\\
%     X-Transformer & 95.75 & 82.46 & 67.22 \\
%     BERT-APLC & 94.49 & 79.74 & 64.46 \\
%     XLNet-APLC & 94.56 & 79.78 & 64.59 \\
%     LightXML & 94.61 & 79.83 & 64.45 \\
%     % attn 1 & 93.00 & 77.85 & 62.94 \\
%     % cls 12 & 94.49 & 79.72 & 64.59 \\
%     % average &  94.74 &  80.32 &  65.18 \\
%     % rank &  94.51 &  80.06 &  64.97 \\
%     % roundrobin &  92.98 &  78.91 &  64.23 \\
%     \end{tabular}
%     \caption{Baseline results on AmazonCat-13K}
%     \label{tab:results}
% \end{table}

\subsection{Retrieval-based Method vs. Representation-based Method}
Although the two models give similar performance on the micro P@k metric, they are based on very different feature and classification algorithms which is not reflected by the metric. In order to show the difference, we use the F1@5 metric evaluated over different bins of labels according to their frequency in the training data. 

The results are shown in Fig. \ref{fig:binned_evaluation}. The horizontal axis represents the label bins according to the number of training instances and the groups are $\{1\sim9, 10\sim 99, \ldots \}$. The vertical axis represents the relative improvement compared with the flat svm baseline. From the figure, we observe that retrieval-based method benefits the lower-frequency (tail) bins, and the representation-based method benefits the high-frequency (head) bins. As most of the training instances concentrate in the head bins, the micro precision metric will be largely impacted by the prediction in those groups. Therefore, the advantage of the retrieval method in the tail bins is shadowed by the micro P@k metric. Especially in the Wiki10-31K dataset, although retrieval based method performs worse on the precision metric, it has a huge advantage on the prediction of tail labels.

\end{comment}






==> tex/informal_theoretical_analysis.tex <==
\section{Theoretical Analyses on the Lower Bound Performance}
Intuitively, our model combines feature from two complementary sources: the corpus specific word importance statistics and neural embedding with word semantics. 
In the theoretical analyses, we demonstrate that our model achieves a lower bound performance as the sparse classifier, given the selected keywords are important and the sparse classifier can separate the positive from the negative instances with non-trivial margin.

Let $\phi_t(\vx)$ be the normalized tf-idf feature vector of text with $\| \phi_t(\vx) \|_2 = 1$. The label embeddings $\{ \vw_1, \ldots, \vw_L \}$ satisfies $\| \vw_i \|_2 \le 1$. In fact, label embeddings can be transformed to satisfy the condition without changing the prediction rank.  

\begin{theorem}[informal]
Let $\vx$ be a text document with tf-idf feature $\phi_t(\vx)$, and $p$ be a positive label and $\sN_p = \{n_1, \ldots, n_{M_p} \}$ be a set of negative labels ranked lower than $p$. Let $\epsilon_i=\mu(\phi_t(\vx), \vv_p, \vv_{n_i})$ and $\epsilon = \min(\{ \epsilon_1, \ldots, \epsilon_{M_p} \})$. An error event $\gE_i$ occurs when $\mu(\mE\phi_t(\vx), \mE \vv_p, \mE\vv_{n_i}) \le 0$. 
The probability of any such error happening satisfies 
\begin{equation}
    P(\gE_1 \cup \ldots \cup \gE_{M_p}) \le 4 {M_p} \exp (-\frac{(\epsilon - \delta)^2d}{50}) 
\end{equation}
When $(\epsilon - \delta) \ge 10 \sqrt{\frac{\log M_p}{d}}$,  $P(\gE_1 \cup \ldots \cup \gE_{M_p})
    \le \frac{1}{M_p}$
\end{theorem}

For each label $l$, the keywords are selected according to importance $\evw_{li}$ of the learned label embedding $\vw_{l}$. Assume a set of keywords $\sK_{w_l}$ is selected, we denote the keyword-selected label embedding as $\vv_l$ where $\evv_{li} = \evw_{li}$ if $i \in \sK_{w_l}$ and $0$ otherwise.

Since both the tf-idf score and the word embedding entries are positive, it is always true that $\langle \phi_t (\vx), \vv_l \rangle \le \langle \phi_t(\vx), \vw_l  \rangle$, with smaller difference when more keywords are selected, especially when all the keywords are kept, $\delta = 0$. We formally define difference between the label embedding $\vw_l$ and the keyword-selected label embedding $\vv_l$.
 
 \begin{definition} 
  For label $l$ and $\delta>0$, the keyword-selected label embedding is $\delta$-bounded if  $\langle \phi_t (\vx), \vv_l \rangle \ge \langle \phi_t(\vx), \vw_l  \rangle - \delta $, the corresponding set of keywords is $\sK_{v_l}^\delta$.
 \end{definition}
 
We define an error margin of prediction between two labels:

 \begin{definition}
 For two labels $p$ and $n$, with text feature $\phi(\vx)$ and the label embeddings $\vw_p, \vw_n$, the error margin is the difference of the predicted score $\mu(\phi (\vx), \vw_p, \vw_n) = \langle \phi (\vx), \vw_p - \vw_n \rangle$. 
 \end{definition}

\begin{lemma} 
Following the notation above, let $\vv$ is the $\delta$-bounded keyword-selected label embedding of $\vw$, then
$
   | \mu( \phi_t(\vx), \vw_p, \vw_n ) 
   - \mu( \phi_t(\vx), \vv_p, \vv_n ) | \le \delta
$
\end{lemma}

Lemma 1 shows that the error margin between the label embedding and the $\delta$-bounded keyword-selected embedding is bounded. All the lemmas and theorems are proved in appendix \ref{appendix:A}.

%To compare the performance of neural model vs. the SVM model, we need a relationship between the feature.
Our goal is to compare the performance between \ourmodel and the SVM model. The \ourmodel model learns dense representations for both the text $\phi_n(\vx) \in \mathbb{R}^d$ and the keywords $\phi_n(\vz_l)$ where $z_{li} \in \sK_{v_l}^\delta$. 
%Although our model uses the BERT model to encode both text representation and label representation, 
Following \citet{luan2020sparse}, we treat $\phi_n(\va) = \mE\va$ as weighted average of word embeddings aggregated by the weights of a sparse vector $\va$, where $\mE \in \mathbb{R}^{d\times v}$ is the word embedding matrix. According to the famous the \textbf{Johnson-Lindenstrauss Lemma}~\citep{johnson1984extensions, ben2002limitations}, even if the entries of $\mE$ are sampled from a random normal distribution $N(0, d^{-1/2})$, with large probability, $\langle \phi_t(\vx), \vv \rangle$ and $\langle \mE\phi_t(\vx), \mE\vv \rangle$ are close.

We formally define an error event when SVM make the correct prediction but the neural model doesn't. If the neural model avoids all such errors, the performance should be at least as good as the SVM model. % An error event made by the neural model is defined as:
%It follows that $\langle \phi_t(\vx), \vw_l - \vw_n \rangle > 0$ If the neural model ranks the negative labels lower, the performance should be bounded by the SVM model.
 %For a given document and a positive label $p$, the score predicted by SVM is $\langle \phi_t(\vx), \vv_p \rangle$ and the score predicted by the neural model is $\langle \mE\phi_t(\vx), \mE\vv_p \rangle$. 
 
\begin{definition} 
Let $p$ be a positive label and $\sN_p = \{n_1, \ldots, n_{M_p} \}$ be the set of negative labels that are ranked below $p$ by SVM. For any negative $n \in \sN_p$, it follows $\mu(\phi_t(\vx), \vw_p, \vw_n) > 0$. An error event $\gE$ occurs when $\mu (\mE \phi_t(\vx), \mE\vv_p, \mE\vv_n) \le 0$.
\end{definition}

The following lemma shows a bound for an error event for a positive label $l$ and a negative label $n \in \sN_l$. 

\begin{lemma}
Let $\vx$ be a text document with tf-idf feature $\phi_t(\vx)$, and $p$ be a positive label and $n\in \sN_p$. Let $\vv_p$ and $\vv_n$ be the $\delta$ bounded keyword label embedding. Assume $\langle \phi_t(\vx), \vv_p - \vv_{n} \rangle = \epsilon$. 
The probability of an error event $\gE$ satisfies $P(\gE) \le 4 \exp (-\frac{(\epsilon - \delta)^2d}{50})$.
\end{lemma}

Lemma 2 models the probability of one error event for label $l$. Using the Union Bound with Lemma 2, we show a bound of probability of all the error events.



\textbf{Discussion:} Theorem 1 shows that the probability of \ourmodel performing worse than the SVM is bounded, especially when $(\epsilon - \delta)$ is larger, the probability is smaller. Intuitively, when $\delta$ is small, it means that the extracted keywords are more meaningful for the SVM model, and thus more informative for our neural encoder. The term $\epsilon$ is taking the mean of error margins $\epsilon_1, \ldots, \epsilon_{M_p}$, which means the model is prone to mistake if the negative labels are indistinguishable from the positive label.  

\textbf{Theoretical analysis vs. the empirical experiments:} We acknowledge the differences between our theoretical analysis and the empirical experiments. First, the bound in the theoretical analysis is very loose as it assumed the word embeddings are random samples from Gaussian distribution. It is shown that the pre-trained language models can produce more meaningful semantic word embeddings based on the context and gain more generalization power. Second, for efficient batch encoding of label keywords, we selected top $k$ keywords for every label, whereas the $\sK_{v_l}^\delta$ is just used for theoretical analysis. The $k$ is a hyper-parameter selected empirically. Lastly, the dual encoder is an additional module on top of the base neural classifier, because encoding the label keywords are beneficially for tail labels, but the head labels can be modeled with the base neural classifier.

==> tex/model.tex <==
\section{Keyword-selected Dual Encoder}
\label{sec:model}
In this section, we proposed a dual encoder framework that leverages the pairs of input document with the pseudo label descriptions extracted from a sparse classifier. We call it the Keyword-selected Dual Encoder (\ourmodelshort).

\noindent \textbf{Sparse classifier:}
We train a linear SVM model with tf-idf feature $\phi_t(\vx)$ as the sparse classifier:
    $$ f_{\text{sparse}}(\vx, l) = \sigma(\langle \phi_t(\vx), \vw_l \rangle)  $$
The learned word embedding $\evw_{li}$ denotes the importance of the word $i$ for label $l$. The top $k$ important keywords selected for label $l$ is denoted as $\vz_l$, where $k$ is a hyperparameter.
% put in implementation details
%We use a different token type embedding for keywords.

\noindent \textbf{KDE:}
We first train a base neural classifier with feature extract $\phi_n(\vx)$ (initialized by BERT) and the label embeddings $\vu_l$ (randomly initialized): 
\begin{equation}
    f_{\text{dense}}(\vx, l) = \sigma(\langle \phi_n(\vx),  \vu_l \rangle)
\end{equation}
Then we fine-tune the model on pseudo label descriptions by sharing the encoder $\phi_n(.)$ for both the text ($\vx$) and keywords ($\vz_l$):
\begin{equation}
    f_{\text{KDE}}(\vx, l) = \frac{\sigma(\langle \phi_n(\vx), \phi_n(\vz_l)\rangle) +  f_{\text{dense}}(\vx, l)}{2}
\end{equation}
The predicted probability is an average of two terms, where $\sigma(\langle \phi_n(\vx), \phi_n(\vz_l)\rangle)$ leverages the document and label semantic matching that benefits the tail label prediction, and $f_{\text{dense}}(\vx, l)$ is a dense classifier that is better optimized for head labels with sufficient training data.

\noindent \textbf{Inference}: we can directly use $f_{\text{KDE}}$ or a weighted sum of sparse and KDE classifiers: 
$$ f_{\text{final}}(\vx, l) = (1-\lambda)f_{\text{sparse}}(\vx, l) + \lambda f_{\text{KDE}} (\vx, l)$$
We set $\lambda = \frac{1}{2}$ as a simple design choice.

\noindent \textbf{Learning:} $f_{\text{dense}}$ and $f_{\text{sparse}}$ are optimized with the BCE loss. For $f_{\text{KDE}}(\vx, l)$, calculating $\phi_n(\vz_l)$ for all labels both expensive and prohibitive by memory limit, so we use negative sampling for in-batch optimization. Specifically, the label representations are calculated over a subset of labels $\sS_b = \sP_b \cup \sN_b$, where $\sP_b$ contains all the positive labels for the instances in the batch and $\sN_b$ are the negative labels with hard negatives and uniform random sampling. For each instance, the hard negative labels are the false positive predictions by the SVM model. The objective for dual encoder is:
\begin{equation}
\begin{split}
    \min \frac{1}{N}\sum_{i=1}^N \Bigg( \Bigg.
    \sum_{p \in \vy_{i}^+} \log f_{\text{KDE}}(\vx, p) \\
    + \sum_{n \in \sS_b \backslash \vy_{i}^+} \log(1 - f_{\text{KDE}}(\vx, n)) \Bigg. \Bigg)
\end{split}
\end{equation}
where $\vy_i^+$ is the set of positive labels for instance $i$.

%Intuitively, our model combines feature from two complementary sources: the corpus specific word importance statistics and neural embedding with word semantics. In the next section, we show a theoretical analysis on the performance on the neural model vs. sparse classifier.



==> tex/motivation.tex <==
%\section{Analysis of Current XMTC Systems}
\section{Rethinking Sparse and Dense XMTC}
\label{sec:rethinking}
Let $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ be the training data where $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{0, 1\}^L$ are the binary ground truth labels.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
Given an instance $\vx$ and a label $l$, a neural classification system jointly learns the feature embedding $\phi_n(\vx; \theta)$ (parameterized by $\theta$) and the label embedding $\vw_l$. The system calculates a relevance score (logits) $s_l = \langle \phi_n(\vx), \vw_l \rangle$, which is then normalized by the sigmoid function to produce $p_l = \sigmoid(s_l)$, indicating the probability of the label being true.
The probability is optimized by the binary cross entropy (BCE) loss:
\begin{equation*}
    \mathcal{L}_{\text{BCE}} = -\sum_{l=1}^L y_l\log p_l + (1-y_l)\log (1-p_l)
\end{equation*}
The derivative of $\mathcal{L}_{\text{BCE}}$ w.r.t the logits is:
\begin{equation*}
    \frac{\partial \mathcal{L}_{\text{BCE}}}{\partial s_l} =
    \begin{cases}
        p_{l} - 1 & \text{if } y_{l}=1 \\
        p_{l} & \text{otherwise} \\
    \end{cases}
\end{equation*}
We analyze the difficulty of both the document and label embedding optimization in the skewed label distribution from the gradient perspective, and show that: 1) the learned document feature lacks for the representation of tail label. 2) the tail label embedding is hard to encode meaningful information by supervised signals alone. We then provide empirical observations together to shed light on our proposed framework.

\subsection{Analysis of Document Feature Learning} 
In multi-label classification, the document feature needs to reflect all the representations of relevant labels. In fact, the gradient describes the relation between feature $\phi_n(\vx)$ and label embedding $\vw_l$. By the chain rule, the gradient of $\mathcal{L}_{\text{BCE}}$ w.r.t the document feature is:
\begin{equation*}
    \frac{\partial \mathcal{L}_{\text{BCE}}(y_{l}, p_{l})}{\partial \phi_n(\vx)} =
    \begin{cases}
        (p_{l} - 1)\vw_l & \text{if } y_{l}=1 \\
        p_{l}\vw_l & \text{otherwise} \\
    \end{cases}
\end{equation*}
By optimizing parameters $\theta$ of feature extractor, 
the document feature is encourage to remove the information of a negative label, that is:
$$\phi_n(\vx; \theta^\prime) \leftarrow \phi_n(\vx; \theta) - \eta p_l \vw_l$$
where $\eta$ is the learning rate.
Since a tail label has an overwhelming number of negative instances and  $\theta$ is shared for all the data, the feature extractor is inclined to remove the tail label information, which will be missing in the document representation. In comparison, the sparse feature like tf-idf is unsupervised from corpus statics, which does not suffer from this problem. The feature may still maintain the representation power to separate the tail labels. 

\subsection{Analysis of Label Feature Learning}
When the labels are treated as indices in a classification system, they are randomly initialized and learned from supervised signals. The gradients of $\mathcal{L}_{\text{BCE}}$ w.r.t the label feature is:
\begin{equation*}
    \frac{\partial \mathcal{L}_{\text{BCE}}(y_{l}, p_{l})}{\partial \vw_l} =
    \begin{cases}
        (p_{l} - 1) \phi_n(\vx) & \text{if } y_{l}=1 \\
        p_{l} \phi_n(\vx) & \text{otherwise} \\
    \end{cases}
\end{equation*}
The label embedding is updated by:
\begin{align*}
    \vw_l^\prime &= \vw_l + \frac{\eta}{N_{\text{train}}}\sum_{i: y_{il} = 1} (1 - p_{il}) \phi_n(\vx_i) \\
    & -\frac{\eta}{N_{\text{train}}} \sum_{i: y_{il}=0} p_{il}\phi_n(\vx_i)
\end{align*}
After the optimization, the label embedding tends to include features from positive instances and exclude features from negative instances. 
As most of the instances are negative for a tail label, the update is inundated with the aggregation of negative features, making it hard to encode distinctive feature reflecting its identity.  
Therefore, learning the tail label embedding from supervised signals alone can be very distracting. Although previous works leverage negative sampling to alleviate the problem~\cite{jiang2021lightxml, chang2020taming},
we argue that it is important to initialize the label embedding with the label side information.

\begin{figure}[th!]
     \centering
     \includegraphics[width=\linewidth]{img/tail_label_example2.png}
     \caption{The evaluation of tail label prediction for SOTA Transformer-based models with macro-averaging F1@k, where $k=19$ for Wiki10-31K and $k=5$ for the other datasets. The figure shows the relative improvement to the SVM baseline with $*$ indicating the significance for $p<0.01$.}
     \label{fig:tail_eval}
\end{figure}


\subsection{Observations and Proposed Idea}
%From the analysis above, it is beneficial for tail label prediction by 1) leveraging the advantage of unsupervised sparse feature, 2) injecting label side information. We provide two related empirical observations to further motivate our proposed framework.

% \begin{table*}[th!]
%     \small
%     \centering
%     \begin{tabular}{l|ccc}
%     \toprule
%     classifier \textbackslash \ characteristics &  & neural \\
%     \hline \\
%   sparse & \makecell{entries are \\ word importance} & abstract semantics \\ 
%     \hline \\
%     neural & unsupervised & supervised \\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparing sparse and dense features.
%     \label{tab:description} }
% \end{table*}


% \begin{table}[th!]
%     \small
%     \centering
%     \begin{tabular}{l|cc}
%     \toprule
%     classifier & sparse & neural \\
%     \hline \\
%     \makecell{label \\embedding} & \makecell{entries are \\ word importance} & abstract semantics \\ 
%     \hline \\
%     \makecell{feature \\embedding} & unsupervised & supervised \\
    
%     \bottomrule
%     \end{tabular}
%     \caption{Comparing sparse and dense features.
%     \label{tab:description} }
% \end{table}
\noindent \textbf{Obs. 1: sparse classifier has an advantage on tail label prediction.}
We evaluate the classification performance of tail labels with less than $10$ training instances by the macro-averaging F1 metric described in \secref{sec:experiment}. In \figref{fig:tail_eval}, the dense models are compared with a linear SVM baseline trained from tf-idf feature, and the relative improvement is reported. The $3$ deep Transformer models except for AttentionXML underperform the sparse classifier on all datasets, with $*$ indicating the significance~\cite{yang1999re} for $p<0.01$. AttentionXML performs the best in two datasets, but it utilizes the more expensive label-word attention that doesn't encode the document into a fixed representation, which we don't seek to improve it in this paper.

\begin{table*}[th!]
    \small
    \centering
    \begin{tabular}{lc|c}
    \toprule
    \bf Dataset & \bf Label Text & \bf Top Keywords \\
    \midrule
    & child care (1) & \makecell{\high{care child parent upbringing family} responsabilitie occupational affordable reconciliation \\ leave reconcile responsibility arise enable need \high{service} effective talent ambition charter} \\
    EURLex-4K & scientific profession (3) & \makecell{\high{science confidential} 452 access society \high{scientific} purposes whose \high{researchers} \\ bodies bank 831 issues may central list recalling \high{data} recognises 412} \\
    & mining extraction(5) & \makecell{ \high{extractive industries extracting drilling} contract soda awarded \high{mineral mining ash} \\ 531 corporation through dialogue tailings communicate tenneco 1600 webb value} \\
    \hline\\
     & phase4 (1) & \makecell{\high{trials} \high{clinical} protection personal directive processed data trial \high{drug} phase eu \\ processing \high{patients} sponsor \high{controller} legislation regulation art investigator \high{study} } \\
   Wiki10-31K & eco-construction (3) & \makecell{\high{solar building cob} passive glazing \high{cordwood thermal timber sewage natural} \\ autonomous \high{roof} \high{clay window insulation} cistern septic shade bale reduce} \\
    & bookmaking (5) & \makecell{ \high{tex book artist} spine \high{binding bind bookbinding bookbinder} nickname scroll \high{signature} \\ someone raise \high{glue sew} texas fold cloth endpaper typeset }\\
    \hline \\
    & booklet envelopes (1) & \makecell{ \high{cabinetmaking booklet} upcoming excerpts building centers \high{cabinet book} joinery \\ kreg mark basics develop provided content \high{produce} allow entire customer \high{covers} } \\
    Amazoncat-13K & sweater dresses (3) & \makecell{favorable \high{slung} impress \high{dye sweater worn} multi \high{dress} pair space \\ super sure palette knit jean low favorite jacket brown \high{soft} }\\
    & farming (5) & \makecell{ \high{crops acres farmers sustainable} hobby \high{grit profitable livestock farms} discusses \\ small issue national gardening \high{soil} readers designed magazine traditional \high{homegrown} } \\
    \bottomrule
    \end{tabular}
    \caption{Example of provided label descriptions with training frequency in parenthesis for the benchmark datasets, and the top $20$ extracted label keywords from the sparse classifier. For illustration purpose, we manually highlight keywords that can enrich the original label text. \label{tab:description} }
\end{table*}
\noindent \textbf{Obs. 2: provided label descriptions are noisy.}
The provided label descriptions are shown in the left of \tblref{tab:description}, which are usually very short, noisy and insufficient to be related to the document with lexical matching. As an example in Wiki10-31K, the label text \textit{phase4} (with only $1$ training instance) is hard even for human to understand the meaning without more context or definitions specific to the document. With generated pseudo label description (explained in the next part), we can understand it is about medical testing phases with keywords \textit{trial, clinical, drug ...} extracted. Although not all the keywords can provide rich semantics to complement the original label text, they may serve as a context for the label to make it more distinguishable, i.e. \textit{responsibility, reconciliation} for label \textit{child care}. 

%\noindent \textbf{Complement neural model with sparse classifier.}
\noindent \textbf{Proposed Idea}
From the analysis of document feature learning and observation 1, the sparse classifier has a strength in tail label prediction. Additionally, the learned label embeddings from a sparse classifier can be interpreted as importance of words in the corpus vocabulary for the label. In this way, we can extract the top k keywords from the label embedding as the pseudo label description. From the analysis of label feature learning, it is important to provide additional label side information for label embedding. In observation 2, the neural model may benefit from the extracted keywords that leverage the knowledge from the sparse classifier and generalize better with neural embeddings of the keywords.

In \secref{sec:model}, we will explain the proposed framework that leverages the pseudo label description; in \secref{sec:theory}, we provide theoretical analysis to relate the performance of our model with respect to the sparse classifier; in \secref{sec:experiment}, we demonstrate the generalization power of our model by experiments on benchmark datasets.

% \begin{enumerate}
% \item Tf-idf is unsupervised which maintains separability even for tail labels, providing better performance on tail label prediction. 
% \item The label embedding of a sparse classifier reflects the token importance, which allows us to extract keywords as pseudo label description. 
% \item Tf-idf and pre-trained neural models provide complementary features, such that tf-idf is corpus specific statistics while neural model reflects general understanding of the language. 
% \item Neural embedding allows the soft semantic matching of the keywords, providing a flexible context compared to hard token matching in sparse classifier.
% \end{enumerate}

%To alleviate the difficulty of optimization of the tail labels, we propose to generate pseudo label description by selecting keywords from a trained sparse classifier with tf-idf feature. 




% We compare the models with two types of features that are frequently used in the classification systems: the tf-idf feature and dense embedding feature.
% \noindent \textbf{Tf-idf+SVM} The one-vs-all linear SVM model is a simple realization of $f(\mathbf{x}, l)$:
% \begin{equation*}
%     f(\vx, l) = \langle \phi_t(\vx), \vw_l \rangle 
% \end{equation*}
% where $\phi_{\text{t}}(\vx) \in \sR^{v}$ converts each text input into the tf-idf feature with vocabulary size of $v$, and $\vw_l \in \mathbb{R}^v$ is the learned parameter of linear classifier for label $l$. The tf-idf feature uses the human defined heuristics to reflect the distributed importance of each word in the training corpus. 

%Although more complicated kernels such as the RBF kernel are introduced in the SVM model for the classification tasks, \cite{chang2011libsvm} shows that a Linear SVM achieves the same performance with a RBF kernel SVM when the feature space is large (refer to Table \ref{tab:dataset} for the number of features in the benchmark datasets). 
%Therefore, we use the Linear SVM to lower computational cost without affecting the performance. 


% The document-vector representation-based methods (\textit{doc-vec}) encodes the raw text into a dense vector representation with neural networks as $\phi_n(\vx)$. %shown in Fig~\figref{fig:method} left.
%Specifically, \citet{liu2017deep} are the first to apply CNN model~\cite{kim-2014-convolutional} to encode the input text $\mathbf{x}$ into a single bottleneck vector as the document-level representation in the XMTC task. Recently, the deep Transformer-based~\cite{NIPS2017_3f5ee243} models quickly exceed the performance of CNN and achieve the state-of-the-art. We choose the deep Transformer-based models and write score function as follows:
% \begin{equation}
%     f(\vx, l) = \langle \phi_n(\vx), \vu_l \rangle 
% \end{equation}
% where $\phi_n(\vx) \in \sR^{d}$ is a $d$ dimensional dense feature usually obtained by the deep transformer models such as BERT~\citep{devlin2018bert} or XLNet~\citep{yang2019xlnet}. 
% $\vu_l$ represents the learned parameter of a linear classifier for label $l$, which is typically optimized by the logistic regression objective $\mathcal{L}_{\mathrm{logistic}}$. We use $\vu_l$ to distinguish from $\vw_l$ because $\vu_l \in \sR^d$ is a compressed dense vector while $\vw_l \in \sR^v$ is sparse ($d \ll v$).






==> tex/theoretical_analysis.tex <==
\section{Theoretical Analysis on Performance}
\label{sec:theory}
In the theoretical analysis, we demonstrate that \ourmodel achieves a lower bound performance as the sparse classifier, given the selected keywords are important and the sparse classifier can separate the positive from the negative instances with non-trivial margin.

Let $\phi_t(\vx)$ be the normalized tf-idf feature vector of text with $\| \phi_t(\vx) \|_2 = 1$. The sparse label embeddings $\{ \vw_1, \ldots, \vw_L \}$ satisfies $\| \vw_l \|_2 \le 1, w_{li} > 0$. In fact, label embeddings can be transformed to satisfy the condition without changing the prediction rank.  
Let $\vz_l$ be the selected keywords and $\vv_l$ be the sparse keyword embedding with $\evv_{li} = \evw_{li}$ if $i$ is keyword and $0$ otherwise. 
We define the keyword importance and error margin which are major terms affecting the performance bound.

 \begin{definition} 
  For label $l$ and $\delta \ge 0$, the sparse keyword embedding is $\delta$-bounded if  $\langle \phi_t (\vx), \vv_l \rangle \ge \langle \phi_t(\vx), \vw_l  \rangle - \delta $. 
 \end{definition}
 
\begin{definition}
 For two labels $p$ and $n$, the error margin is the difference between the predicted scores $\mu(\phi (\vx), \vw_p, \vw_n) = \langle \phi (\vx), \vw_p - \vw_n \rangle$. 
\end{definition}
 
We state the theorem below with additional assumptions and proofs in appendix \ref{appendix:A}.

\begin{theorem}
\label{th:main}
Let $\phi_t(\vx)$ and $\phi_n(\vx)$ be the sparse and dense (dimension $d$) feature, $\vw_l$ be the label embedding and  $\vz_l$ be the $\delta$-bounded keywords. For a positive label $p$, let $\sN_p = \{n_1, \ldots, n_{M_p} \}$ be a set of negative labels ranked lower than $p$. 
The error margin $\epsilon_i=\mu(\phi_t(\vx), \vw_p, \vw_{n_i})$ and $\epsilon = \min(\{ \epsilon_1, \ldots, \epsilon_{M_p} \})$. An error event $\gE_i$ occurs when $\mu(\phi_n(\vx), \phi_n(\vz_p), \phi_n(\vz_{n_i}) ) \le 0$. 
The probability of any such error happening satisfies 
\begin{equation*}
    P(\gE_1 \cup \ldots \cup \gE_{M_p}) \le 4 {M_p} \exp (-\frac{(\epsilon - \delta)^2d}{50}) 
\end{equation*}
When $(\epsilon - \delta) \ge 10 \sqrt{\frac{\log M_p}{d}}$, the probability is bounded by $\frac{1}{M_p}$.
% \begin{equation*}
%     P(\gE_1 \cup \ldots \cup \gE_{M_p})
%     \le \frac{1}{M_p}
% \end{equation*}
\end{theorem}

\noindent \textbf{Discussion:} 
An error event occurs when the sparse model makes a correct prediction but the neural model doesn't. If the neural model avoids all such errors, the performance should be at least as good as the SVM model, and Theorem \ref{th:main} gives a bound of that probability.

The term $\delta$ measures the importance of selected keywords (smaller the more important), the term $\epsilon$ term measures the error margin of the correctly predicted positive and negative pairs by the sparse model. The theorem states that the model achieves a lower bound performance as sparse classifier if the keywords are informative and error margin is non-trivial.

\noindent \textbf{Theoretical analysis vs. empirical experiments:} 
1) the bound in the theoretical analysis is very loose as the proof doesn't consider contextualized semantic embedding of Transformer models, which could produce more meaningful features based on the context and generalize better. 2) we select top $k$ keywords for every label as a hyper-parameter for efficient batch encoding of label keywords instead of the $\delta$-bounded keywords. 3) by mining hard negatives as inputs to \ourmodel, the neural model may generalize better to avoid the mistakes by sparse classifier.
%The reason is that encoding the label keywords are beneficially for tail labels, but the head labels can be modeled with the base neural classifier.

==> tex/tmp.tex <==
\subsection{Preliminary}
%\section{One-vs-all Multi-label Classification}
%We will introduce the task and notation in Section \ref{sec:background_intro}, the SOTA methods under evaluation in Section \ref{sec:background_methods} and the evaluation metrics in Section \ref{sec:background_metric}. 

Let $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ be the training data where $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
% We denote a training dataset with $N_{\text{train}}$ instances and $L$ labels as 
% $\train=\{\left(\mathbf{x}_i, \mathbf{y}_i\right)_{i=1}^{N_{\text{train}}} \}$ such that $\mathbf{x}_i$ is the input text and $\mathbf{y}_i\in\{-1, +1\}^L$ is the ground truth label list.
%
The XMTC method can be formulated as learning a scoring function $f(\mathbf{x}, l) \in \sR$ defined on an input and candidate label pair $(\vx, l)$. The score should be higher for relevant labels than irrelevant labels.
The objective function of a classification model is defined as:
%Then we can define a classification model with the following objective function:
%The one-vs-all classifiers is optimized by:
\begin{equation*}
        \min_{f} \quad \frac{1}{N_{\text{train}} L} \sum_{i=1}^{N_{\text{train}}} \sum_{l=1}^{L} \mathcal{L}(y_{i l}, f(\mathbf{x}_i, l))
\end{equation*}
where $\mathcal{L}(\cdot, \cdot)$ is an instance-wise loss, such as a hinge loss in a Linear SVM or a sigmoid loss in the final layer of a neural network.

In the evaluation, since multi-labels can be relevant for an input document $\mathbf{x}$, a typical way is to measure the quality of a top-k ranked list of the predicted label: \begin{equation}
    \operatorname{Top-k}([f(\vx, 1), \ldots, f(\vx, L)])
\end{equation}
% \begin{equation*}
%         \mathbf{p}^k = \operatorname{Top-k}([f(\mathbf{x}, 1), \ldots, f(\mathbf{x}, L)])
% \end{equation*}


% We should add to related work later
%Although these approaches achieve good performance, with the enormous label space, these methods suffer from huge computational burden.As a remedy, Tree-based approaches are proposed ~\cite{fastxml,parabel,khandagale2019bonsai} to partition the labels into several clusters hierarchically based on their positive instances or correlations.Cluster-level classifiers are trained at each tree layer, which allows prediction in a hierarchical order. Many recent neural models are built upon tree-based methods, in which $f$ is neural networks.


\subsection{Motivation 1. Sparse vs. Dense Classifier} 
We compare the models with two types of features that are frequently used in the classification systems: the tf-idf feature and dense embedding feature.
\noindent \textbf{Tf-idf+SVM} The one-vs-all linear SVM model is a simple realization of $f(\mathbf{x}, l)$:
\begin{equation*}
    f(\vx, l) = \langle \phi_t(\vx), \vw_l \rangle 
\end{equation*}
where $\phi_{\text{t}}(\vx) \in \sR^{v}$ converts each text input into the tf-idf feature with vocabulary size of $v$, and $\vw_l \in \mathbb{R}^v$ is the learned parameter of linear classifier for label $l$. The tf-idf feature uses the human defined heuristics to reflect the distributed importance of each word in the training corpus. 

%Although more complicated kernels such as the RBF kernel are introduced in the SVM model for the classification tasks, \cite{chang2011libsvm} shows that a Linear SVM achieves the same performance with a RBF kernel SVM when the feature space is large (refer to Table \ref{tab:dataset} for the number of features in the benchmark datasets). 
%Therefore, we use the Linear SVM to lower computational cost without affecting the performance. 


The document-vector representation-based methods (\textit{doc-vec}) encodes the raw text into a dense vector representation with neural networks as $\phi_n(\vx)$. %shown in Fig~\figref{fig:method} left.
%Specifically, \citet{liu2017deep} are the first to apply CNN model~\cite{kim-2014-convolutional} to encode the input text $\mathbf{x}$ into a single bottleneck vector as the document-level representation in the XMTC task. Recently, the deep Transformer-based~\cite{NIPS2017_3f5ee243} models quickly exceed the performance of CNN and achieve the state-of-the-art. We choose the deep Transformer-based models and write score function as follows:
\begin{equation}
    f(\vx, l) = \langle \phi_n(\vx), \vu_l \rangle 
\end{equation}
where $\phi_n(\vx) \in \sR^{d}$ is a $d$ dimensional dense feature usually obtained by the deep transformer models such as BERT~\citep{devlin2018bert} or XLNet~\citep{yang2019xlnet}. 
$\vu_l$ represents the learned parameter of a linear classifier for label $l$, which is typically optimized by the logistic regression objective $\mathcal{L}_{\mathrm{logistic}}$. We use $\vu_l$ to distinguish from $\vw_l$ because $\vu_l \in \sR^d$ is a compressed dense vector while $\vw_l \in \sR^v$ is sparse ($d \ll v$).
%From another point of view, it computes the similarity between the document vector and label embeddings as a score for the label. 
%The predicted labels are ranked according to the probability, and the top labels are compared against the ground truth label list. 

%The most representative deep Transformer-based models tailored for the XMTC task are  X-transformer~\cite{chang2020taming}, APLC-XLNet~\cite{ye2020pretrained} and LightXML~\cite{jiang2021lightxml}, which are discussed in Appendix~\ref{sec:append_experiment}.

%The tf-idf is distributional statistics which reflects the word importance in a corpus, and the dense embedding feature re

We highlight the key differences between the two types of features: 1) tf-idf is corpus dependent and the neural embedding reflects the general language understanding. 2) tf-idf is unsupervised but the neural embedding is supervised. 3) the tf-idf is a sparse vector but the dense embedding is not.

. Dense vectors are effective for
encoding local syntactic and semantic cues leveraging recent advances in contextualized text encoding (Devlin et al., 2019), while sparse vectors
are superior at encoding precise lexical information.

\section{Evaluation Methodology}
\label{sec:background_metric}
A typical way to evaluate XMTC is to measure the quality of the label ranked list produced by the model.
The micro-based metrics takes average over all the test instances:
\begin{equation}
    \operatorname{Micro@k}  = \frac{1}{N_{\text{test}}} \sum_{i=1}^{N_{\text{test}}} \operatorname{Metric}(\mathbf{p}_i^k,\mathbf{y}_i)
\end{equation}
where $N_{\text{test}}$ is the number of test instances and $\mathbf{p}^k_i, \mathbf{y}_i$ are the predicted top $k$ ranked list and the ground truth labels respectively. 
$\operatorname{Metric}$ is a function to score the quality of the ranked list such as P@k (Precision at k)~\cite{liu2017deep, you2018attentionxml, parabel, khandagale2019bonsai, ye2020pretrained, chang2020taming, jiang2021lightxml}, R@k (Recall at k), N@k (Normalized Discounted Cumulative Gain at k)~\cite{fastxml} , or PSP@k (Propensity-scored Performance at k)~\cite{PSP}, which are discussed in Section \ref{sec:append_micro_eval}.

In this paper, we report the micro F1@k as the evaluation metric, which is calculated by:
\begin{equation}
    \operatorname{F1@k} = 2 \frac{P@k \cdot R@k }{P@k + R@k }
\end{equation}

\paragraph{Macro-averaging Metrics}
For better evaluation on the label level, we proposed to apply the \textit{macro-averaging F1} metric, where the performance score on each label is given an equal weight when calculating the average.
Moreover, the macro-averaging F1 metric can be applied to groups of labels according to their training frequency to clearly reflect the performance on head labels and tail labels. We call this metric the \textit{binned macro-averaging F1} metric.
Let $L_b$ be a group of labels, then the macro-based F1 on $L_b$ is calculated by:
\begin{equation}
    \operatorname{Macro@k} = \frac{1}{|L_b|} \sum_{l \in L_b} \operatorname{F1}_l^k
\end{equation}
where $L_b$ is the label set for bin $b$ and $\operatorname{F1}_l^k$ is the $\operatorname{F1}$ metric for label $l$ evaluated on top $k$ ranked list $\mathbf{p}^k$.

Specifically, the F1@k for label $l$ over predicted ranked list $\mathbf{p}^k$ is calculated according to the confusion matrix at Table \ref{tab:confusion_matrix}:
\begin{equation*}
    \mathrm{P}^k_{l}= \frac{\mathrm{TP}_l^k}{\mathrm{TP}_l^k + \mathrm{FP}_l^k} ,\quad \mathrm{R}^k_{l}=\frac{\mathrm{TP}_l^k}{\mathrm{TP}_l^k + \mathrm{FN}_l^k} ,\quad
    \mathrm{F1}^k_l=  2\frac{\mathrm{P}^k_l \cdot \mathrm{R}^k_l}{\mathrm{P}^k_l+ \mathrm{R}^k_l}
\end{equation*}

% \begin{align*}
%     \mathrm{P}^k_{l}= \frac{\mathrm{TP}_l^k}{\mathrm{TP}_l^k + \mathrm{FP}_l^k} &,\quad \mathrm{R}^k_{l}=\frac{\mathrm{TP}_l^k}{\mathrm{TP}_l^k + \mathrm{FN}_l^k} \\
%     \mathrm{F1}^k_l= & 2\frac{\mathrm{P}^k_l \cdot \mathrm{R}^k_l}{\mathrm{P}^k_l+ \mathrm{R}^k_l}
% \end{align*}
where $\mathrm{P}^k_l, \mathrm{R}^k_{l}, \mathrm{F1}^k_l$ are the precision, recall, F1 at $k$ for label $l$. As a designed choice, we set $\mathrm{F1}^k_l = 0$ if a label $l$ is never predicted.
%Note that for tail labels, the total prediction (TP+FP) is usually very small or even zero because tails labels are treated as negative labels most of the time, which makes models tend to give these labels a small probability. 

\begin{table}[h!]
    \centering
    \small
    \caption{Confusion Matrix for label $l$ and top $k$ ranked list $\mathbf{p}^k$.}
    \begin{tabular}{c|cc}
    & $l$ in $\mathbf{y}$ & $l$ not in $\mathbf{y}$ \\
    \hline
    $l$ in $\mathbf{p}^k$ & True Positive($\mathrm{TP}_l^k$) & False Positive($\mathrm{FP}_l^k$) \\
    $l$ not in $\mathbf{p}^k$ & False Negative($\mathrm{FN}_l^k$) & True Negative($\mathrm{TN}_l^k$) \\
    \end{tabular}
    \vspace{-1.0em}
    \label{tab:confusion_matrix}
\end{table}


==> tex/tmp_theoretical.tex <==
\section{Theoretical Analyses on the Lower Bound Performance}
Intuitively, our model combines feature from two complementary sources: the corpus specific word importance and neural embedding with word semantics. In the theoretical analyses, we demonstrate that our model achieves a lower bound performance as the sparse classifier, given the selected keywords are important and the sparse classifier can separate the positive from the negative instances with non-trivial margin.

\textbf{Notations:} Let $\phi_t(\vx)$ be the normalized tf-idf feature vector of text, s.t. $\| \phi_t(\vx) \|_2 = 1$. We assume that the label embeddings $\{ \vw_1, \ldots, \vw_L \}$ satisfies $\| \vw_i \|_2 \le 1$ and $ \evw_{ij} \ge 0, i\in\{1, \ldots, L\}, j\in \{1, \ldots, V\}$. In fact, since we use a ranking metric, we can always normalize the label embeddings by 
$\frac{\vw_l - \min( \{\evw_{ij}\} )}{\max  (\{ \| \vw_i - \min( \{\evw_{ij}\} ) \|_2 \}) }$,
without changing the prediction rank.  

For each label $l$, the keywords are selected according to importance $\evw_{li}$ of the learned label embedding $\vw_{l}$. Assume a set of keywords $\sK_{w_l}$ is selected, we denote the keyword-selected label embedding as $\vv_l$ where $\evv_{li} = \evw_{li}$ if $i \in \sK_{w_l}$ and $0$ otherwise.

Since both the tf-idf score and the word embedding entries are positive, it is always true that $\langle \phi_t (\vx), \vv_l \rangle \le \langle \phi_t(\vx), \vw_l  \rangle$, with smaller difference when more keywords are selected, especially when all the keywords are kept, $\delta = 0$. We formally define difference between the label embedding $\vw_l$ and the keyword-selected label embedding $\vv_l$.
 
 \begin{definition} 
  For label $l$ and $\delta>0$, the keyword-selected label embedding is $\delta$-bounded if  $\langle \phi_t (\vx), \vv_l \rangle \ge \langle \phi_t(\vx), \vw_l  \rangle - \delta $, the corresponding set of keywords is $\sK_{v_l}^\delta$.
 \end{definition}
 
We define an error margin of prediction between two labels:

 \begin{definition}
 For two labels $p$ and $n$, with text feature $\phi(\vx)$ and the label embeddings $\vw_p, \vw_n$, the error margin is the difference of the predicted score $\mu(\phi (\vx), \vw_p, \vw_n) = \langle \phi (\vx), \vw_p - \vw_n \rangle$. 
 \end{definition}

\begin{lemma} 
Following the notation above, let $\vv$ is the $\delta$-bounded keyword-selected label embedding of $\vw$, then
$
   | \mu( \phi_t(\vx), \vw_p, \vw_n ) 
   - \mu( \phi_t(\vx), \vv_p, \vv_n ) | \le \delta
$
\end{lemma}

Lemma 1 shows that the error margin between the label embedding and the $\delta$-bounded keyword-selected embedding is bounded. All the lemmas and theorems are proved in appendix \ref{appendix:A}.

%To compare the performance of neural model vs. the SVM model, we need a relationship between the feature.
Our goal is to compare the performance between \ourmodel and the SVM model. The \ourmodel model learns dense representations for both the text $\phi_n(\vx) \in \mathbb{R}^d$ and the keywords $\phi_n(\vz_l)$ where $z_{li} \in \sK_{v_l}^\delta$. 
%Although our model uses the BERT model to encode both text representation and label representation, 
Following \citet{luan2020sparse}, we treat $\phi_n(\va) = \mE\va$ as weighted average of word embeddings aggregated by the weights of a sparse vector $\va$, where $\mE \in \mathbb{R}^{d\times v}$ is the word embedding matrix. According to the famous the \textbf{Johnson-Lindenstrauss Lemma}~\citep{johnson1984extensions, ben2002limitations}, even if the entries of $\mE$ are sampled from a random normal distribution $N(0, d^{-1/2})$, with large probability, $\langle \phi_t(\vx), \vv \rangle$ and $\langle \mE\phi_t(\vx), \mE\vv \rangle$ are close.

We formally define an error event when SVM make the correct prediction but the neural model doesn't. If the neural model avoids all such errors, the performance should be at least as good as the SVM model. % An error event made by the neural model is defined as:
%It follows that $\langle \phi_t(\vx), \vw_l - \vw_n \rangle > 0$ If the neural model ranks the negative labels lower, the performance should be bounded by the SVM model.
 %For a given document and a positive label $p$, the score predicted by SVM is $\langle \phi_t(\vx), \vv_p \rangle$ and the score predicted by the neural model is $\langle \mE\phi_t(\vx), \mE\vv_p \rangle$. 
 
\begin{definition} 
Let $p$ be a positive label and $\sN_p = \{n_1, \ldots, n_{M_p} \}$ be the set of negative labels that are ranked below $p$ by SVM. For any negative $n \in \sN_p$, it follows $\mu(\phi_t(\vx), \vw_p, \vw_n) > 0$. An error event $\gE$ occurs when $\mu (\mE \phi_t(\vx), \mE\vv_p, \mE\vv_n) \le 0$.
\end{definition}

The following lemma shows a bound for an error event for a positive label $l$ and a negative label $n \in \sN_l$. 

\begin{lemma}
Let $\vx$ be a text document with tf-idf feature $\phi_t(\vx)$, and $p$ be a positive label and $n\in \sN_p$. Let $\vv_p$ and $\vv_n$ be the $\delta$ bounded keyword label embedding. Assume $\langle \phi_t(\vx), \vv_p - \vv_{n} \rangle = \epsilon$. 
The probability of an error event $\gE$ satisfies $P(\gE) \le 4 \exp (-\frac{(\epsilon - \delta)^2d}{50})$.
\end{lemma}

Lemma 2 models the probability of one error event for label $l$. Using the Union Bound with Lemma 2, we show a bound of probability of all the error events.

\begin{theorem}
Let $\vx$ be a text document with tf-idf feature $\phi_t(\vx)$, and $p$ be a positive label and $\sN_p = \{n_1, \ldots, n_{M_p} \}$ be a set of negative labels ranked lower than $p$. Let $\epsilon_i=\mu(\phi_t(\vx), \vv_p, \vv_{n_i})$ and $\epsilon = \min(\{ \epsilon_1, \ldots, \epsilon_{M_p} \})$. An error event $\gE_i$ occurs when $\mu(\mE\phi_t(\vx), \mE \vv_p, \mE\vv_{n_i}) \le 0$. 
The probability of any such error happening satisfies 
\begin{equation}
    P(\gE_1 \cup \ldots \cup \gE_{M_p}) \le 4 {M_p} \exp (-\frac{(\epsilon - \delta)^2d}{50}) 
\end{equation}
When $(\epsilon - \delta) \ge 10 \sqrt{\frac{\log M_p}{d}}$,  $P(\gE_1 \cup \ldots \cup \gE_{M_p})
    \le \frac{1}{M_p}$
\end{theorem}

\textbf{Discussion:} Theorem 1 shows that the probability of \ourmodel performing worse than the SVM is bounded, especially when $(\epsilon - \delta)$ is larger, the probability is smaller. Intuitively, when $\delta$ is small, it means that the extracted keywords are more meaningful for the SVM model, and thus more informative for our neural encoder. The term $\epsilon$ is taking the mean of error margins $\epsilon_1, \ldots, \epsilon_{M_p}$, which means the model is prone to mistake if the negative labels are indistinguishable from the positive label.  

\textbf{Theoretical analysis vs. the empirical experiments:} We acknowledge the differences between our theoretical analysis and the empirical experiments. First, the bound in the theoretical analysis is very loose as it assumed the word embeddings are random samples from Gaussian distribution. It is shown that the pre-trained language models can produce more meaningful semantic word embeddings based on the context and gain more generalization power. Second, for efficient batch encoding of label keywords, we selected top $k$ keywords for every label, whereas the $\sK_{v_l}^\delta$ is just used for theoretical analysis. The $k$ is a hyper-parameter selected empirically. Lastly, the dual encoder is an additional module on top of the base neural classifier, because encoding the label keywords are beneficially for tail labels, but the head labels can be modeled with the base neural classifier.
